Summarize and Generate to Back-translate: Unsupervised Translation of Programming Languages

Back-translation is widely known for its effectiveness in neural machine translation when there is little to no parallel data. In this approach, a source-to-target model is coupled with a target-to-source model trained in parallel. The target-to-source model generates noisy sources, while the source-to-target model is trained to reconstruct the targets and vice versa. Recent developments of multilingual pre-trained sequence-to-sequence models for programming languages have been very effective for a broad spectrum of downstream software engineering tasks. Hence, training them to build programming language translation systems via back-translation is compelling. However, these models cannot be further trained via back-translation since they learn to output sequences in the same language as the inputs during pre-training. As an alternative, we propose performing back-translation via code summarization and generation. In code summarization, a model learns to generate natural language (NL) summaries given code snippets. In code generation, the model learns to do the opposite. Therefore, target-to-source generation in back-translation can be viewed as a target-to-NL-to-source generation. We show that our proposed approach performs competitively with state-of-the-art methods. We have made the code publicly available.

==> [EACL 2023] Summarize Generate to Backtranslate/figures/qual_exam.tex <==
\begin{figure}[t]
% \rule{\linewidth}{0.6pt}
\centering
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Input in Java}
\end{center}
\vspace{-5pt}
\begin{tabular}{@{}l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public static boolean generator(PsiBuilder b, int l){
    boolean r = false;
    if(!recursion_guard(b, l)) return r;
    r = generator_0(b, l + 1);
    if(!r) return generator_1(b, l + 1);
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\\
\vspace{5pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
%  (w/o fine-tuning)
\begin{center}
    \underline{\normalsize (1) Java to Python Generation}
\end{center}
\vspace{-5pt}
\begin{tabular}{@{}l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=4
        \color{red!10}
    \fi
    }
]
public static boolean generator(PsiBuilder b, int l){
    boolean r = false;
    if(!recursion_guard(b, l)) return r;
    if(!generator_0(b, l)) return r;
    r = generator_0(b, l + 1);
    if(!r) return generator_1(b, l + 1);
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\\
% \vspace{5pt}
% \begin{center}
%     \normalsize{\color{blue} Summarize and Generate to Back-translate}
% \end{center}
% \vspace{10pt}
% \rule{\linewidth}{0.6pt}
\begin{center}
    \underline{\normalsize (2) Java Code to NL Summary}
\end{center} 
\vspace{-7pt}
\begin{flushleft}
guard is used to determine if a generator is already defined .
\end{flushleft}
% \vspace{5pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{\normalsize (3) NL Summary to Python Code}
\end{center} 
\vspace{-5pt}
\begin{tabular}{@{}l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}
def is_generator(self, name):
    if name in self._generators:
        return True
    if name in self._generators[name]:
        return True
    return False
\end{lstlisting}
\end{tabular}
\end{adjustbox}
% \vspace{-1mm}
\caption{
Although PLBART is asked to generate in Python given input in Java (1), it generates in Java (due to its pre-training objective). In contrast, PLBART, fine-tuned on code summarization and generation, generates ``noisy'' translations (as in (2, 3)).
}
% \vspace{-2mm}
\label{fig:qual_ex1}
\end{figure}


==> [EACL 2023] Summarize Generate to Backtranslate/figures/tsne_example.tex <==
\begin{figure*}[t]
	\centering
	\subfloat[PLBART \label{sfig:plbart}]{%
		\includegraphics[width=0.49\textwidth]{images/plbart.png}
	}
	\subfloat[PLBART + \sng \label{sfig:plbart_msg}]{%
		\includegraphics[width=0.49\textwidth]{images/plbart_msg.png}
	}
% 	\vspace{-2mm}
	\caption{T-SNE plot of function embeddings of Java and Python functions. \Cref{sfig:plbart} shows the embedding generated by the PLBART model. 
	\Cref{sfig:plbart_msg} are the generated embedding when the PLBART is finetuned to jointly summarize code to NL and generate code from NL (PLBART + \sng). 
% 	The average distance between parallel java and python code is 343.01 as generated by PGLM and 230.74 as generated by PGLM + S\&G.
    While PLBART clusters programs from each PLs, parallel programs in different PLs are brought closer to each other by PLBART + \sng.
	}
	\label{fig:tsne}
% 	\vspace{-2mm}
\end{figure*}

==> [EACL 2023] Summarize Generate to Backtranslate/sections/0_abstract.tex <==
\begin{abstract}
Back-translation is widely known for its effectiveness in neural machine translation when there is little to no parallel data. In this approach, a source-to-target model is coupled with a target-to-source model trained in parallel. The target-to-source model generates noisy sources, while the source-to-target model is trained to reconstruct the targets and vice versa. Recent developments of multilingual pre-trained sequence-to-sequence models for programming languages have been very effective for a broad spectrum of downstream software engineering tasks. Hence, training them to build programming language translation systems via back-translation is compelling. However, these models cannot be further trained via back-translation since they learn to output sequences in the same language as the inputs during pre-training. As an alternative, we propose performing back-translation via code summarization and generation. In code summarization, a model learns to generate natural language (NL) summaries given code snippets. In code generation, the model learns to do the opposite. Therefore, target-to-source generation in back-translation can be viewed as a \emph{target-to-NL-to-source} generation. We show that our proposed approach performs competitively with state-of-the-art methods.
We have made the code publicly available.\footnote{\url{https://github.com/wasiahmad/SumGenToBT}}

% We take advantage of labeled data for the code summarization task. 
% , if not exceeding their translation performance between Java and Python languages.
% In back-translation, a target-to-source model generates noisy sequences in the source language and a source-to-target model is trained to reconstruct the original sequences in the target language.
% Back-translation uses a target-to-source model to generate noisy sources and trains a source-to-target model to reconstruct the targets.  
% Recently, \emph{TrasnCoder}, an unsupervised programming language translation model, is trained jointly via denoising autoencoding (DAE) and back-translation.



% Programming language translation can be viewed as a two step process: (1) code to natural language (NL) summary generation (target-to-NL), and (2) NL summary to code generation (NL-to-source).


% In code summarization, a model learns to generate a natural language (NL) summary given a piece of code (target-to-NL), and in code generation, the model learns to do the opposite (NL-to-source). 
% We propose to perform back-translation from target-to-source programming language via target-to-summary and summary-to-source generation. We take advantage of the availability of labeled data for the code summarization task. We show that our proposed framework performs comparably to TransCoder, if not, exceeds its performance in programming language translation between Java and Python.

% existing sequence-to-sequence language models pre-trained via DAE cannot be further trained via back-translation to learn programming language translation. 
% Existing sequence-to-sequence language models pre-trained via denoising autoencoding (DAE) or fill-in-the-blank
% Our study suggests existing sequence-to-sequence language models pre-trained via DAE cannot be further trained via back-translation to learn programming language translation. 
% This is because the models learn to generate output sequences in the same language as the inputs during pre-training. 

\end{abstract}




==> [EACL 2023] Summarize Generate to Backtranslate/sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

The choice of programming language (PL) in software development depends on the requirement of the software and the available features of a particular PL. In modern API-driven software development, language choice often depends on the availability of libraries and APIs.
The advent of newer and richer programming languages often requires legacy software to be translated into modernized PLs. 
In theory, modern programming languages' ``Turing Completeness'' allows rule-based translation of programs from one PL to another. 
The rule-based translation may require an extensive number of custom-written transformation rules and could end up producing very unreadable source code. In addition, such a translation could entail translating the entire library, even if a library implementing similar functionality is available in the target PL.  

\input{figures/qual_exam}
\input{figures/tsne_example}

Aligning libraries and APIs across different PLs is a non-trivial task. Recent progress in Neural Machine Translation (NMT) \cite{bahdanau2014neural, vaswani2017attention} leveraging pre-trained models~\cite{feng-etal-2020-codebert, guo2020graphcodebert, roziere2021dobf, ding2021contrastive,ahmad-etal-2021-unified, wang-etal-2021-codet5} could be a possible way to learn the alignment between PLs and translate source code across languages.
% demonstrated program understanding~\cite{} and generation capacity~\cite{}. 
% However, the NMT models should exhibit a profound understanding of the source language and a reasonably well generation capacity to translate programs across languages. There are several recently proposed pretrained models that demonstrated program understanding~\cite{feng-etal-2020-codebert, guo2020graphcodebert, roziere2021dobf, ding2021contrastive} and generation capacity~\cite{ahmad-etal-2021-unified, wang-etal-2021-codet5}.

A significant challenge in supervised learning for NMT is the need for large-scale parallel corpora. 
For instance, if we are planning to train a translator for {\tt Java} to {\tt Python} translation, we need a considerable number of the same program (\emph{i.e.}, exhibiting the same semantic behavior) in both languages. Availability of such parallel datasets is a vital challenge in programming language translation~\cite{chen2018tree}. Back-Translation (BT)~\cite{edunov-etal-2018-understanding, lachaux2020unsupervised} is a clever way to learn alignments across different languages.
While BT demonstrates success in NMT, those require either (i.) small (perhaps noisy) parallel datasets or (ii.) a model with some capacity of cross-lingual generation - to kickstart the BT-based learning process.

In this work, we investigate the suitability of the multilingual Pre-trained Sequence-to-Sequence Model (PSM) 
% (\emph{e.g.}, PLBART~\cite{ahmad-etal-2021-unified}) 
for unsupervised programming language translation via BT. In particular, we assume a use-case scenario where {\em no} parallel data is available. Without much of a surprise, we empirically found that, while these PSMs are good at generating code in each language, they exhibit very little to no knowledge about cross-lingual generation since such PSMs are typically trained to reconstruct code sequences from noisy inputs.
For example, when we provide the input code in \Cref{fig:qual_ex1} to PLBART~\cite{ahmad-etal-2021-unified} and ask to generate Python code without training, it generates a slight variation of the input Java code, showing its lack of knowledge about cross-lingual generation.


To endow such PSMs with knowledge about cross-lingual generation, we propose using a third language ({\em i.e.}, English).
Since a large quantity of monolingual code corpora comes with documentation, which supposedly describes what the source code is doing, we train a Summarize-and-Generate (\sng) model that can generate pseudo-parallel code sequences.
\Cref{fig:qual_ex1} shows PLBART's behavior when it is further trained via \sng. First, given the Java code, it generates an NL summary (\cref{fig:qual_ex1}-2) and subsequently generates Python Code (\cref{fig:qual_ex1}-3). 
We empirically show that, even if such \sng model generates noisy parallel sequences, it allows us to employ PSMs in the BT-based training to learn programming language translation.
% it significantly improves the translation performance of PSMs using BT.


In summary, we present a Summarize-and-Generate (\sng) based approach to enable unsupervised program translation training of PLBART via Back-Translation (BT).
% of pretrained sequence-to-sequence source code models.
% (\eg PLBART~\cite{ahmad-etal-2021-unified}). 
Experiment results show that our proposed approach makes PLBART
% pre-trained sequence-to-sequence model 
trainable via BT and performs competitively with state-of-the-art program translation models.

% \footnote{We have made our code publicly available at \url{https://github.com/hidden/hidden}.}
% https://github.com/wasiahmad/SumGenToBT
% \url{https://github.com/hidden/hidden}.}
% In-depth analysis shows that with \sng training, PLBART performs comparably or better than state-of-the-art unsupervised program translator.



==> [EACL 2023] Summarize Generate to Backtranslate/sections/2_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.85\textwidth]{images/overview.pdf}
%     \caption{
%         Overview of our proposed back-translation framework to train PLBART. In the first $m$ steps (out of total $N$ training steps), we use a multilingual code summarization and generation model ($\mathcal{S}, \mathcal{G}$) to perform back-translation. In the remaining steps ($N-m$), PLBART is trained via standard back-translation method.
%     }
%     \label{fig:overview}
% \end{figure*}

\begin{figure*}[t]
	\centering
    \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/Step1.pdf}
    \caption{Step1: Supervised training of PLBART on Code Summarization and Generation (\sng).}
    \label{sfig:overview-s-n-g}
    \end{subfigure}
    
    \vspace{10pt}
    
    \begin{subfigure}{0.90\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/Step2.pdf}
    \vspace{-2mm}
    \caption{Step2: Unsupervised training of PLBART via Backtranslation (BT). In the first $m$ training steps (out of total $N$ steps), PLBART generates natural language (NL) summary of the code in target language (Python in this example) and generates the code in source language (Java in this example) from the NL summary. In the remaining $N-m$ steps, PLBART directly generates the code in source language from the code in target language.}
    \label{sfig:overview-bt}
    \end{subfigure}
	\caption{Overview of our proposed framework to train PLBART in two sequential steps.
	}
	\label{fig:overview}
\end{figure*}



Recent years saw several Pre-trained Sequence-to-Sequence models (PSM) \cite{ahmad-etal-2021-unified, wang-etal-2021-codet5}. These models are pre-trained on hundreds of Gigabytes of source code. Thus, in this work, we are motivated to investigate their adoption in learning program translation via back-translation.
% in the back-translation approach. In particular, we investigate whether we can directly train these pre-trained models for program translation via back-translation. 
To understand such feasibility, we investigate the program representations generated by the PSM. 
% As a case study, we chose PLBART \cite{ahmad-etal-2021-unified}. 
% Motivated by Tatoeba \cite{artetxe-schwenk-2019-massively} for understanding representation learning behavior of multilingual models, 
% we probe into the function embeddings given by PSMs.
As a case study, we chose PLBART \cite{ahmad-etal-2021-unified} and evaluated its multilingual embeddings as suggested in \citet{artetxe-schwenk-2019-massively}.
% Motivated by Tatoeba \cite{artetxe-schwenk-2019-massively} for understanding representation learning behavior of multilingual models, we probe into the function embeddings given by PSMs.
We find the parallel Java function for each of the 948 Python functions using the parallel dataset proposed in \citet{lachaux2020unsupervised}.
We find the nearest neighbor using cosine similarity between function embeddings and calculate the error rate.
Unsurprisingly, PLBART performs poorly in function retrieval with an 87.5\% error rate.
% Without much of a surprise, we find that in {\em only 12.5\%} cases (top-1 retrieval accuracy),
% \footnote{top-1 retrieval accuracy.} 
% the closest function is the corresponding Java function.

In comparison, we fine-tune PLBART jointly on code summarization and generation in Java and Python. 
Repeating the experiment of function retrieval, we find that fine-tuned PLBART's error rate drops to 23.7\%.
To visually illustrate the embeddings produced by PLBART and its fine-tuned variant, we provide a T-SNE plot of 8 sample functions' embedding in Figure \ref{fig:tsne}.
We see the functions that belong to the same language are clustered together while the same functions in two different languages are far apart from each other (see \Cref{sfig:plbart}).

% , which shows programs in the same language are clustered together. The embeddings of the same function in different languages are far apart. 

In contrast, the fine-tuned PLBART breaks up the intra-language clusters and brings functions in different languages close to each other in the embedding space (see \Cref{sfig:plbart_msg}).
These results motivate us to initialize the translation models with fine-tuned PLBART on code summarization and generation for back-translation as it learned some alignment across programming languages.

% These results suggest that fine-tuned PLBART on code summarization and generation learns some alignment across programming languages, which we consider as motivation to kickstart the back-translation by initializing the translation models with fine-tuned PLBART.

% We further train the PSM to simultaneously Summarize-and-Generate (\sng) and repeat our previous experiment on understanding the program embedding. After \sng training, the PSM generated embedding brings  {\em 76.3\%} programs from different languages to be the closest to each other. As shown in \cref{sfig:plbart_msg}, \sng training breaks up the intra-language clusters learned by PSM and brings programs in different languages close to each other. We also observe a similar trend when finding the closest python function given the java function embeddings. Nevertheless, since \sng training endows PSM with some initial alignment across languages, we are motivated to use \sng trained PSM to kickstart the back-translation. 



==> [EACL 2023] Summarize Generate to Backtranslate/sections/3_method.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.85\textwidth]{images/overview.pdf}
%     % \vspace{-2mm}
%     \caption{
%     Overview of our proposed back-translation framework to train PLBART. In the first $m$ steps (out of total $N$ training steps), we use a multilingual code summarization and generation model ($\mathcal{S}, \mathcal{G}$) to perform back-translation. In the remaining steps ($N-m$), PLBART is trained via standard back-translation method.
%     }
%     % \vspace{-2mm}
%     \label{fig:overview}
% \end{figure*}
%  Figure has been moved to mid of the motivation section. 

\section{Approach}
\label{sec:method}

% \notewa{One of our NAACL reviewers said, ``this section reads in a round-about way, starting with defining back-translation, and then code summarization and generation, and then back-translation again. It will read better if they start with detailing their code summarization and generation and then followed by how they use this model fine-tuned for code summarization and generation to do back-translation; instead of repeating the back-translation description twice. Another aspect that can be improved is in terms of notation. In Section 3, all the equations have consistently referred to source code as x and target code as y. However, the algorithm section (Algorithm 1) uses different notations $\_s$ or $\_t$ (for source and target, consecutively -- with $x$ and $y$ used interchangeably). This has made the reading of the Algorithm difficult and inconsistent with the in-text equations (eq. 1 and eq. 3). If the authors can make the notation in Algorithm 1 more consistent with the equations, that will improve readability greatly.''}


Sequence-to-sequence models, such as PLBART \cite{ahmad-etal-2021-unified}, CodeT5 \cite{wang-etal-2021-codet5}, SPT-Code~\cite{niu2022spt} map source code sequences into a shared multilingual space by pre-training on multiple programming languages jointly using unlabeled data ({\em e.g.}, source code from Github).
% due to jointly pre-training in many languages
The pre-training objective of these models is either denoising autoencoding (DAE) or fill-in-the-blank, where the models reconstruct the original code snippet or predict the missing code tokens given a corrupted code snippet. Although pre-trained jointly on many languages, these models only learn to generate in the same language as input.
% \footnote{For example, given a code snippet in Java language as input and setting ``<python>'' as the decoder prefix token (language ID), PLBART still generates code in Java.}
As a result, these models are not trainable via back-translation (BT) to learn programming language translation in an unsupervised fashion.
As an alternative, we propose translating to and from natural language to perform back-translation between two programming languages. We refer to translating to and from natural language as code summarization and code generation, respectively.
Our proposal is motivated based on the availability of \emph{bimodal} data, source code, and their summaries that are used to train code summarization and generation models.

% In this section, we review the back-translation approach (\cref{sec:bt}), and then describe the multilingual training scheme for code summarization and generation (\cref{sec:sum_gen}). Finally, we detail our approach, summarize--generate to back-translate (\cref{sec:sum_gen_as_bt}).


\subsection{Code Summarization and Generation}
\label{sec:sum_gen}
Source code documentation (\eg docstring or comment) written by software developers is available along with source code on a large scale. Such documentation has been the key source to form code summarization datasets \cite{wan2018improving, hu2018summarizing, leclair-mcmillan-2019-recommendations, husain2019codesearchnet},
% These datasets are also utilized 
and to study natural language (NL) to code generation~\cite{parvez-etal-2021-retrieval-augmented}. 
It is tangible that we can use a code summarization and generation model to translate programming languages. 
% In particular, we envision the natural language as a bridge between programming languages. 
Such a model would first generate an NL summary from an input code in the source language and then generate code from the previously generated NL summary in the target language. As we show in the evaluation, such an approach does not work well in practice (see \cref{table:main_result}); however, code summarization and generation models are viable proxies to generate noisy translations. This enables us to train PLBART, to begin with generating noisy translations, and further learn to improve in a self-supervised fashion when trained via back-translation.
Formally, we jointly train PLBART in a supervised setting to learn code summarization ($\mathcal{S}$) and generation ($\mathcal{G}$):
% using labeled paired data:
\begin{align}
\label{eq:mulsumgen}
\begin{split}
    \mathcal{S} &= TRAIN^{\text{Code} \rightarrow \text{Summary}} \left(\mathcal{P}_{c, s} \right) \\
    \mathcal{G} &= TRAIN^{\text{Summary} \rightarrow \text{Code}} \left(\mathcal{P}_{c, s} \right)
\end{split}
\end{align}
where $\mathcal{P}_{c, s}$ is estimated using the code-to-text benchmark from CodeXGlue \cite{CodeXGLUE}. We follow \citet{tang-etal-2021-multilingual} to perform multilingual fine-tuning of PLBART (in Java and Python) to learn $\mathcal{S}$ and $\mathcal{G}$.
% \footnote{\url{https://github.com/wasiahmad/PLBART/tree/main/multilingual}}
% In the following section, we detail our proposed approach.



\subsection{Back-translation}
\label{sec:bt}
Back-translation (BT) is one of the most popular ways for unsupervised machine translation \cite{artetxe2017unsupervised, lample2018unsupervised, lample-etal-2018-phrase}.
In this approach, we leverage monolingual data in an unsupervised fashion.
% According to the BT approach, 
BT jointly trains a source-to-target model coupled with a backward target-to-source model. 
% trained in parallel
The target-to-source model translates target sequences into the source language, producing noisy sources corresponding to the ground truth target sequences. The source-to-target model is then trained to generate the targets from the noisy sources and vice versa. The two models are trained in parallel until convergence. This training procedure is widely known as \emph{online back-translation} and is the focus of this work.


Back-translation uses a target-to-source model to generate noisy sources and trains a source-to-target model to reconstruct the targets. Specifically, in each step $k$ (a mini-batch update), back-translation performs the following:
\begin{align}
\label{eq:bt}
\begin{split}
    \mathcal{P}_k^{(f)} &= \left\{ (x, f_{k-1} (x)) | x \in \mathcal{D}_{\text{source}} \right\} \\
    b_{k} &= TRAIN^{\text{target} \rightarrow \text{source}} \left(\mathcal{P}_k^{(f)}\right) \\
    \mathcal{P}_k^{(b)} &= \left\{ \left(b_k(y), y\right) | y \in \mathcal{D}_{\text{target}} \right\} \\
    f_{k} &= TRAIN^{\text{source} \rightarrow \text{target}} \left( \mathcal{P}_k^{(b)} \right).
\end{split}
\end{align}
Here, $\mathcal{D}_{source}$, $\mathcal{D}_{target}$ represents unlabeled  data in source and target languages and $TRAIN$ indicates standard sequence-to-sequence training.

Generally, the training via back-translation starts from a forward ($f_0$) and a backward ($b_0$)  model that is trained using parallel data (small gold-standard or large-scale but noisy). Then an extensive collection of unlabeled data is used to train the translation models.
In this work, we assume there is \emph{no} parallel data available across programming languages.
We initialize the forward and backward model with the pre-trained language model, PLBART.
As mentioned before, PLBART cannot generate code in a language different from the input (not even a noisy code) (for example, \cref{fig:qual_ex1}-1).
Therefore, we propose jointly fine-tuning PLBART on code summarization and generation on multiple programming languages in a supervised setting.
Then use the resulting model to initialize the forward and backward model ($f_0$, $b_0$) for back-translation.




\subsection{Summarize--Generate to Back-translate}
\label{sec:sum_gen_as_bt}

% The back-translation method requires the \emph{target-to-source} ($b$) and \emph{source-to-target} ($f$) models to generate semantically equivalent (parallel) sequences in the source and target languages, respectively. 
% These parallel sequences are then used to train the models to learn translations as described in Eq. \eqref{eq:bt}.
% Specifically, the parallel sequences $\{(\hat{x}, y), (x, \hat{y})\}$ created by computing $\hat{y} \leftarrow f_{k-1}(x)$ and $\hat{x} \leftarrow b_k(y)$ kick-start the learning process in back-translation.
% Generally, the curated parallel sequences tend to be noisy since we do not have access to accurate {target-to-source} and {source-to-target} models. 
% However, both the models trained in parallel via back-translation until convergence, resulting in useful translation models.

The recent advancements of pre-trained sequence-to-sequence models on programming languages enables us to use them in initializing the {source-to-target} ($f$) and {target-to-source} ($b$) models for back-translation. Presumably, such pre-trained models should facilitate the learning process during training. 
% Still, they are unable to generate code snippets across languages (as shown in Figure \ref{fig:qual_ex1}) due to their pre-training objective, \ie reconstruction of targets from the noisy sources.
Yet, their pre-training objective -- \ie reconstruction of original input from a noisy source limits their ability to generate code snippets across languages (as shown in \Cref{fig:qual_ex1}).
For example, PLBART as $f(\cdot)$ and $b(\cdot)$ would reconstruct the input, resulting in $f_{k-1}(x) \approx x$ and $b_k(y) \approx y$. 
As a result, the models will learn to merely copy the input sequences rather than translate them.

% In the back-translation method, the \emph{source-to-target} and \emph{target-to-source} models can be initialized from pre-trained sequence-to-sequence models, \eg PLBART. 
% However, due to their inability to generate code across languages (as shown in Figure \ref{fig:qual_ex1}), their direct utilization results in unsuccessful back-translation training. 
% Specifically, PLBART as $f(\cdot)$ and $b(\cdot)$ (shown in Eq. \eqref{eq:bt}) attempts to reconstruct the input, resulting in $f_{k-1}(x) \approx x$ and $b_k(y) \approx y$ that allows the model to copy input rather than to learn translation.
% Therefore, we propose to make use of annotated parallel data between programming and natural languages to fine-tune PLBART and then use its parameters to initialize \emph{source-to-target} and \emph{target-to-source} models for back-translation.

To this end, we propose to make use of available parallel data between programming and natural languages to fine-tune PLBART and then use its parameters to initialize {source-to-target} ($f$) and {target-to-source} ($b$) models for back-translation.
Consequently, we revise the back-translation training method outlined in Eq. \eqref{eq:bt} to follow a \emph{two-step generation} process to perform back-translation: code-to-summary generation in natural language followed by summary-to-code generation in the source language.
Formally, the first $m$ steps (while $k \leq m$) of back-translation is performed as:
\begin{align}
\label{eq:sgb}
\begin{split}
    \mathcal{P}_k^{(f)} &= \left\{ \left(x, {\mathcal{G}\left(\mathcal{S}\left(x\right)\right)}\right) | x \in \mathcal{D}_{\text{source}} \right\} \\
    % b_{k} &= TRAIN^{\text{target} \rightarrow \text{source}} \left(\mathcal{P}_k^{(f)}\right) \\
    \mathcal{P}_k^{(b)} &= \left\{ \left({ \mathcal{G}\left(\mathcal{S}\left(y\right)\right)}, y\right) | y \in \mathcal{D}_{\text{target}} \right\}.
    % \\
    % f_{k} &= TRAIN^{\text{source} \rightarrow \text{target}} \left( \mathcal{P}_k^{(b)} \right).
\end{split}
\end{align}

% The difference between Eq \eqref{eq:bt} and \eqref{eq:sgb} is highlighted in blue.
We find the noisy parallel sequences\footnote{The output sequences are still noisy since the code summarization and generation models are not highly accurate although trained in a supervised fashion.} 
% $\{\left(x, {\color{blue}\mathcal{G}\left(\mathcal{S}\left(x\right)\right)}\right), \left({\color{blue}\mathcal{G}\left(\mathcal{S}\left(x\right)\right)}, y\right)\}$ 
generated via summarization and generation commences the learning process.
% After $m$ steps, back-translation is performed as shown in Eq. \eqref{eq:bt}.
% We find this simple trick allows PLBART to translate target code into ``noisy'' sources that commences the learning process.
The overall idea of our proposed framework is illustrated in Figure \ref{fig:overview} and the Algorithm \ref{alg:sgb} describes the training procedure.
Note that we find it is sufficient to apply our proposed summarization-generation based back-translation only for the first $m$ steps as the {source-to-target} and {target-to-source} models gradually learn to translate, the standard back-translation training reinstated.


\begin{algorithm}[t]
% \renewcommand{\thealgorithm}{}
% \small
\caption{Training Procedure}
{\bf Input:} 
% Parallel data $\mathcal{D}_{(s, nl)}$ and $\mathcal{D}_{(t, nl)}$ between programming languages $s$, $t$ and natural language $nl$; 
Monolingual (unlabeled) data $\mathcal{D}_{source}$ and $\mathcal{D}_{target}$; number of initial steps $m$; number of total steps $I$; code summarizer $\mathcal{S}(\cdot,\cdot)$; code generator $\mathcal{G}(\cdot,\cdot)$; parameters $\theta$ to initialize the forward and backward translation models $f(\cdot,\cdot)$ and $b(\cdot,\cdot)$. \\
{\bf Output:} Final model parameters $\theta$.
\begin{algorithmic}[1]
% \Require
\For{$k = 0,\cdots,I$}
    % \State $y_s \leftarrow$ Sample a batch from $\mathcal{D}_s$
    % \State $y_t \leftarrow$ Sample a batch from $\mathcal{D}_t$
    \State $y \leftarrow (y_s \sim\mathcal{D}_{source}) \cup (y_t \sim\mathcal{D}_{target}$)
    \If{$k \leq m$}
        % \State $\hat{x}_s \sim \mathcal{G}_{\theta}(\cdot|\mathcal{S}_{\theta}( \cdot|y_t))$\
        % \State $\hat{x}_t \sim \mathcal{G}_{\theta}(\cdot|\mathcal{S}_{\theta}(\cdot|y_s))$
        \State $x_{nl} \sim \mathcal{S}(\cdot|y)$ \Comment{code-to-summary}
        \State $\hat{x} \sim \mathcal{G}(\cdot|x_{nl})$
        \Comment{summary-to-code}
    \Else
        % \State $\hat{x}_s \sim b_{\theta}(\cdot | y_t)$
        % \State $\hat{x}_t \sim f_{\theta}(\cdot | y_s)$
        \State $\hat{x} \leftarrow (x_s \sim b(\cdot|y_t)) \cup (x_t \sim f(\cdot|y_s))$ 
        % \Comment{Back-translation}
    \EndIf
    % \State $\mathcal{B} \leftarrow \{\langle \hat{x}_s, y_t\rangle\} \cup \{\langle \hat{x}_t, y_s\rangle\}$
    \State Update $\theta$ by maximizing log-likelihood of $f(\hat{x}_s, y_t)$ and $b(\hat{x}_t, y_s)$
    % and $b_{\theta}(\hat{x}_t, y_s)$
\EndFor
\end{algorithmic}
\label{alg:sgb}
\end{algorithm}



% In this work, we apply our proposed framework to build translation system in Java and Python programming languages.

% \paragraph{Python-to-Java translation}
% \begin{align}
% \begin{split}
%      \mathcal{P}_k^{(\mathcal{S},\ \mathcal{G})} &= \left\{ \left(\mathcal{G}\left(\mathcal{S}\left(y\right)\right), y\right)\ |\ y \in \mathcal{D}_{\text{Java}} \right\} \\
%     b_{k} &= TRAIN^{\text{Python} \rightarrow \text{Java}} \left( \mathcal{P}_k^{(\mathcal{S},\ \mathcal{G})} \right).
% \end{split}
% \end{align}


% \paragraph{Java-to-Python translation}
% \begin{align}
% \begin{split}
%     \mathcal{P}_k^{(\mathcal{S},\ \mathcal{G})} &= \left\{ \left(\mathcal{G}\left(\mathcal{S}\left(y\right)\right), y\right)\ |\ y \in \mathcal{D}_{\text{Python}} \right\} \\
%     f_{k} &= TRAIN^{\text{Java} \rightarrow \text{Python}} \left( \mathcal{P}_k^{(\mathcal{S},\ \mathcal{G})} \right).
% \end{split}
% \end{align}


==> [EACL 2023] Summarize Generate to Backtranslate/sections/4_exp_setup.tex <==
\section{Experiment Setup}


\subsection{Models and Baselines}

\paragraph{Our model} 
% As noted earlier, PLBART \cite{ahmad-etal-2021-unified} and CodeT5 \cite{wang-etal-2021-codet5} are two popular sequence-to-sequence models pre-trained on source code that cannot be trained via back-translation (BT). As an alternative, our proposed approach can be leveraged to train both models to learn programming language translation in an unsupervised fashion. In this work, we chose PLBART to perform experiments and show the effectiveness of our proposed approach.
Our proposed approach can be applied to pre-trained sequence-to-sequence models, \eg PLBART \cite{ahmad-etal-2021-unified} and CodeT5 \cite{wang-etal-2021-codet5}. In this work, we chose PLBART\footnote{Since its pretraining implementation is publicly available at \url{https://github.com/wasiahmad/PLBART}.} to perform experiments and show the effectiveness of our proposed framework.

\subsection*{Baseline Models}
We compare our proposed approach applied to PLBART with the following existing approaches.
 
% \smallskip
% \noindent$\bullet$~\textbf{j2py \hspace{0.5em}}
\paragraph{j2py} 
is a framework that translates Java source code to Python.\footnote{\url{https://github.com/natural/java2python}} 
It follows handwritten rules manually built using expert knowledge.

% \smallskip
% \noindent$\bullet$~\textbf{Summarize-and-Generate ($\mathcal{S} \& \mathcal{G}$) \hspace{0.5em}}
\paragraph{Summarize-and-Generate ($\mathcal{S} \& \mathcal{G}$)}
performs code-to-code translation via two steps, code-to-summary and summary-to-code generation. We evaluate the $\mathcal{S} \& \mathcal{G}$ model (as in Eq. \eqref{eq:mulsumgen}) that is used to perform code summarization and generation in our proposed framework to train PLBART via BT.

% \noindent$\bullet$~\textbf{TransCoder}
\paragraph{TransCoder} 
% \smallskip
% \noindent$\bullet$~\textbf{TransCoder \hspace{0.5em}} 
is a neural translation model for programming languages \cite{lachaux2020unsupervised}. TransCoder is developed by pretraining Transformer \cite{vaswani2017attention} via masked language modeling (MLM) objective \cite{devlin2018bert} on monolingual source code datasets. In a second step, TransCoder is trained via denoising autoencoding (DAE) and BT. In this work, we consider TransCoder as the \textbf{primary} baseline.\footnote{We compare TransCoder and PLBART in terms of model architecture and training setup in the Appendix D.}

% \notewa{We should mention the differences between PLBART and TransCoder to highlight, why their comparison is not fair.}

\paragraph{DOBF}
% \smallskip
% \noindent$\bullet$~\textbf{DOBF \hspace{0.5em}} 
\citet{roziere2021dobf} proposed a pretraining objective, DOBF, that leverages the structural aspects of programming languages. According to this pretraining paradigm, the identifiers (class, function, and variable names) in code snippets are obfuscated, and a model is trained to recover the original names. DOBF shares the same neural architecture as TransCoder. We report the evaluation performances of TransCoder and DOBF from the official code release by \citet{lachaux2020unsupervised}.\footnote{ \url{https://github.com/facebookresearch/CodeGen/blob/main/docs/transcoder.md\#results}).}

\input{table/1_data_stat}


\subsection{Evaluation Dataset and Metrics}

\paragraph{Evaluation Dataset}
\citet{lachaux2020unsupervised} proposed an evaluation dataset composed of parallel functions in Java, Python, and C++ languages. The dataset consists of 464 Java to Python and 482 Python to Java test examples, with 10 unit test cases accompanying each.

\subsection*{Evaluation Metrics}


\paragraph{BLEU}
% \noindent$\bullet$~\textbf{BLEU \hspace{0.5em}} 
measures n-gram overlap between a generated translation and a collection of reference translations \cite{papineni-etal-2002-bleu}.

% \smallskip
% \noindent$\bullet$~\textbf{Exact Match (EM) \hspace{0.5em}} 
\paragraph{Exact Match (EM)} 
represents the percentage of generated translations exactly match with the collection of reference translations. 

% \smallskip
% \noindent$\bullet$~\textbf{CodeBLEU \hspace{0.5em}} 
\paragraph{CodeBLEU}
% \notewa{adding definition of CodeBLEU will probably help.}
measures grammatical and logical correctness in addition to n-gram overlap between generated and reference translations \cite{ren2020codebleu}. 
% CodeBLEU assesses grammatical and logical correctness based on the abstract syntax tree and the data-flow structure.
CodeBLEU is defined as a weighted sum of n-gram match, weighted n-gram match,\footnote{ Different weights are assigned to n-grams such that the keywords (\eg \texttt{for}, \texttt{while}) have higher weights} syntax match (based on AST), and data-flow match.

% \smallskip
% \noindent$\bullet$~\textbf{Computational Accuracy (CA) \hspace{0.5em}} 
\paragraph{Computational Accuracy (CA),} proposed by \citet{lachaux2020unsupervised}, assess functional correctness; a translated code is considered correct if it passes a set of unit tests. 
It evaluates if a generated function outputs the same as the reference when given the same set of inputs. This metric overcomes the shortcoming of match-based metrics (\eg BLEU, CodeBLEU) by accounting for the program-execution behavior \cite{lachaux2020unsupervised,chen2021evaluating}. 
% Several recent works \cite{lachaux2020unsupervised,chen2021evaluating} showed that match-based metrics (\eg BLEU, CodeBLEU) are unable to account for the large and complex space of programs functionally equivalent to a reference solution.
% \citet{lachaux2020unsupervised} introduced this evaluation
%  to assess functional correctness; a translated code is considered correct if it passes a set of unit tests.
% perform evaluation based on unit tests. 

\input{table/2_main_result}


\subsection{Training Datasets and Preprocessing}
\label{subsec:dataset}

\paragraph{Code Summarization and Generation} \citet{CodeXGLUE} curated a code summarization dataset consisting of code and summary pairs based on the CodeSearchNet dataset \cite{husain2019codesearchnet}. We use this dataset in Java and Python programming languages to train the code-to-summary and summary-to-code generation models.

\paragraph{Back-translation (BT)}

For BT training (as discussed in \cref{sec:sum_gen_as_bt}), we use the GitHub public dataset available on Google BigQuery \cite{hoffa2016github}.\footnote{\url{https://console.cloud.google.com/marketplace/product/github/github-repos}} 
We first deduplicate\footnote{We used a hash-based data deduplication method.} the GitHub dataset at the program level, extract the functions, and finally perform another deduplication at the function level. 
% This dataset is also used to pre-train PLBART and TransCoder.
Note that the Github dataset is composed of source code that covers a wide variety of programming topics (as they come from various projects). In contrast, the evaluation dataset is composed of programming problems covering basic data structure and algorithmic concepts. Therefore, to investigate the impact of data on BT training, we alternatively chose \emph{unparallel} code samples in Java and Python from CodeNet \cite{puri2021project}. The CodeNet dataset is collected from two online judge websites, \emph{AIZU Online Judge} and \emph{AtCoder}, and composed of submissions for 4053 problems. We use the deduplicated accepted solutions to the problems for BT training. Presumably, CodeNet and the evaluation dataset \cite{lachaux2020unsupervised} have a similar nature that should positively impact downstream translation performance.

% \footnote{\url{https://onlinejudge.u-aizu.ac.jp}} and AtCoder\footnote{\url{https://atcoder.jp}}.



% \paragraph{Github}
% \noindent$\bullet$~\textbf{Github} 


% \smallskip
% \noindent$\bullet$~\textbf{CodeNet} 
% \paragraph{CodeNet} 



\paragraph{Preprocessing}
We use \texttt{tree\_sitter}\footnote{\url{https://github.com/tree-sitter}} for tokenizing Java functions and the tokenizer of the standard library for Python.\footnote{\url{https://docs.python.org/3/library/tokenize.html}}
We extract standalone functions\footnote{Standalone functions can be used without instantiating a class. In Java, this corresponds to static methods, and in Python, it corresponds to functions outside classes.} from the BT training datasets following the function extraction technique from \citet{lachaux2020unsupervised}.
Considering our computational budget, we filter the standalone functions exceeding a maximum length of 256 to cope with our computational resources.
The statistics of the preprocessed datasets are presented in Table \ref{table:data_stat}.

% For preprocessing source code, we use the publicly available source code of TransCoder \cite{lachaux2020unsupervised}.\footnote{https://github.com/facebookresearch/CodeGen}



\subsection{Implementation Details}
We jointly train PLBART on code summarization and generation in Java and Python using the authors' provided code.\footnote{\url{https://github.com/wasiahmad/PLBART/tree/main/multilingual}}
Subsequently, we train PLBART via back-translation as described in Algorithm \ref{alg:sgb}. We set $I = 10,000$ and tuned $m = 200$.\footnote{We tuned $m$ in the range [100, 1000] with 100 steps.}
% proposed in this work for a maximum of 10,000 steps with 100 warm-up steps.
We train PLBART using 8 Nvidia GeForce RTX 2080 Ti GPUs, and the effective batch size is maintained at 1024 instances at both training stages. 
We optimize PLBART with the Adam optimizer \cite{kingma2014adam}, a learning rate of 10e-4, and use a polynomial learning rate decay scheduling.
The best models are selected based on the validation BLEU scores.
We implement our approach in Fairseq~\cite{ott-etal-2019-fairseq} and use float16 operations to speed up training.

% \footnote{\url{https://github.com/wasiahmad/PLBART}}

\paragraph{Decoding}
During inference, we use beam search decoding \cite{koen-2004-pharaoh} to generate multiple translations using PLBART. We chose greedy search (Beam 1) as the \emph{default} decoding scheme for validation and evaluation.
However, following \citet{lachaux2020unsupervised}, we report two sets of results for the computational accuracy (CA) metric: CA@n B=n, the percentage of functions with at least one correct translation in the beam (of size n), and CA@1 B=n the percentage of functions where the hypothesis in the beam with the highest log-probability is a correct translation.




==> [EACL 2023] Summarize Generate to Backtranslate/sections/5_results.tex <==
\section{Results and Analysis}
% We aim to address the following questions.
% \begin{compactenum}
%     \item Does our proposed approach empowers PLBART to learn programming language translation? (\cref{sec:main_result})
%     \item Does summarization and generation enable us to create parallel examples to warmup PLBART for back-translation? (\cref{sec:analysis1})
%     \item Does the use of in-domain data (CodeNet) in training lead to better translations? (\cref{sec:analysis2})
% \end{compactenum}

\input{table/3_beam_result}


\subsection{Main Result}
\label{sec:main_result}

\Cref{table:main_result} shows the performance of our proposed approach and the baseline models on both Java to Python and Python to Java translation. 
We begin by comparing PLBART directly used in back-translation (BT) training with our proposed approach (the last block in \Cref{table:main_result}). 
Since PLBART does not know to generate across languages, when the model is trained via BT, it only learns to copy the input sources. As a result, PLBART scores 0\% EM and 0\% CA, while 30+ BLEU and CodeBLEU scores.
In contrast, following our proposed approach of summarizing and generating to back-translate, PLBART trained via BT (via \sng) achieves 40.4\% and 31.9\% CA scores.
This performance is competitive to state-of-the-art translation system, TransCoder.\footnote{Note that, while comparing PLBART with TransCoder on the translation performance, their differences (shown in \Cref{table:replication_params}) should be taken into consideration.}
We compare them using beam search decoding in \Cref{table:beam_result}.


\input{appendix/table/2_checkpoint_eval}
\input{table/7_data_impact}


% The primary objective of this work is to study the feasibility of using pre-trained sequence-to-sequence models for unsupervised programming language translation via BT. 
% The experimental results conclude that such models cannot directly be used in BT training; however, training via \sng empowers them to generate across languages and further be trained via BT to learn to translate.
Overall, the experimental results confirm our conjecture that pre-trained sequence-to-sequence models cannot be effectively used in BT training; however, training via \sng empowers them to generate across languages and be further trained via BT to learn programming language translation.

% indicate that they are not a reliable indicator of translation correctness.
% \footnote{Several recent works \cite{kulal2019spoc,lachaux2020unsupervised,chen2021evaluating} showed that match-based metrics (\eg BLEU, CodeBLEU) are unable to account for the large and complex space of programs functionally equivalent to a reference solution.} 
% \notewa{Can we clarify further?}

% Although PLBART is a multi-lingual model pre-trained to generate code, it does not work well when directly trained with back translation, as evident by the result (0\% EM and 0\% CA). We attribute such poor performance to PLBART's lack of knowledge about cross-lingual alignment. pre-trained Multi-Lingual Sequence to Sequence Source Code Models such as PLBART, as is, cannot translate across languages without further training.
% We also show the performance of a PLBART model trained via Back-Translation.
% Finally, we show the empirical results of the PLBART model, which is first trained to Summarize and Generate and then trained via Back-Translation (BT). 

% Note that, PLBART lags comparing to DOBF on Java to Python translation as DOBF has shown to perform better on downstream tasks due to its pre-training objective.
% The results suggest that while \sng and PLBART trained via BT does not produce useful translations, PLBART trained via BT initialized from \sng capable to perform translation.


\subsection{Analysis}

\paragraph{Summarize and generate to create parallel data}
% \label{sec:analysis1}
Our proposed approach generates parallel code sequences on the fly (online) for training. An alternative to our approach is to use a code summarization and generation model to create parallel code sequences (offline) and warm-start PLBART for back-translation-based training. We compare these two approaches in \Cref{table:checkpoint_impact}, and the results show that both approaches perform comparably.
However, it is essential to note that the online setting gives us flexibility as we can tune the number of initial steps ($m$ in Algorithm \ref{alg:sgb}).
In contrast, the offline setting requires generating a sufficiently large number of parallel code sequences for effective training.


% \repeatit[5]{Placeholder\par}

\paragraph{Impact of in-domain training data}
% \label{sec:analysis2}
The evaluation dataset comprises solutions to programming problems involving data structures and algorithm concepts. While Github offers large-scale unlabeled data, most of its code belongs to software projects that use APIs and advanced functionalities. Therefore, we utilize an alternative dataset called CodeNet collected from two online judge websites. We refer to this dataset as \emph{in-domain} since its nature aligns with the evaluation dataset (data structure and algorithm focused problems aggregated from GeeksforGeeks).
We compare in-domain data usage with Github data on BT-based training.
The results in \Cref{table:data_impact} show that the use of in-domain data significantly boosts the performance in both translation directions.
A detailed error analysis reveals that such a performance boost is due to a reduction in {\tt TypeError}. 
We speculate that in-domain data have similarities in the data type usage that helps the model.
% Due to the page limit, we present more findings of the error analysis and qualitative examples in the Appendix.
We present further error analysis and qualitative examples in the Appendix.
% In addition, we discuss the limitations and risks of using our proposed model in the Appendix.
% In addition, we perform a rigorous error analysis to show the strength and weaknesses of PLBART-based translation model. 

% \input{figures/example1}

% \paragraph{Qualitative Examples}
% \Cref{fig:example1} shows an example of Java-to-Python translation by PLBART. The translated code is both syntactically and semantically correct \ie our compiler could successfully parse and build the translated code. It passed 2 test cases out of 10 when executed. The translated code is slightly different from the input Java code. In particular, line 13 in the input Java code is a loop that iterates backward (decreasing order). However, line 12 in the generated python code iterates forward (increasing order). 
% If the generated python code was {\tt range(c-1, 0, -1)} instead of {\tt range(c-1)}, it would pass all the test cases. 
% We attribute such behavior to the fact that {\tt range(*)} is much more frequent pattern than {\tt range(*, 0, -1)} in python code.

% We provide more analysis in Appendix.


==> [EACL 2023] Summarize Generate to Backtranslate/sections/6_relwork.tex <==
\section{Related Work}

% \subsection{Programming Language Translation}
\paragraph{Programming Language Translation}
% \noindent\textbf{Programming Language Translation \hspace{0.5em}}
Translating programs or source code across different programming languages (PL) requires a profound understanding of the PLs. Having strictly defined syntax and semantics, PLs are suitable for phrase-based statistical machine translation~\cite{nguyen2013lexical, karaivanov2014phrase, aggarwal2015using}. 
\citet{chen2018tree} introduced a tree-to-tree machine translation to translate programs and to learn the syntactic alignment between source and target PL. Recently proposed pre-trained programming language models showed promising results in translating programs across PLs~\cite{feng2020codebert, guo2020graphcodebert, ahmad-etal-2021-unified, ahmad2021avatar}. However, these approaches require a set of parallel programs to train the encoder-decoder model.

Recently proposed Transcoder \cite{lachaux2020unsupervised} shows initial success results in unsupervised program translation, eliminating the requirement of bi-modal data. They achieve such jointly training a model using XLM~\cite{NIPS2019_8928}, Denoising Auto Encoding (DAE)~\cite{vincent2008extracting}, and Back-Translation(BT)~\cite{lample2018unsupervised}. This work empirically investigated the suitability of adopting BT to train existing pre-trained encoder-decoder models and proposed an alternative via summarization and generation.

% \notewa{We want to discuss prior works as in Section 2 of this paper \cite{roziere2021leveraging} on ``Translation of Programming Languages''.}

% \subsection{Unsupervised Machine Translation via Back-translation}

% \vspace{-4pt}
\paragraph{Unsupervised Machine Translation via Back-translation}
% \smallskip
% \noindent\textbf{Unsupervised Machine Translation via Back-translation \hspace{0.5em}}
Gathering sufficiently large parallel corpora has been a significant challenge for Machine Translation (MT)~\cite{guzman-etal-2019-flores}. Several research efforts are invested in learning MT using monolingual data~\cite{artetxe-etal-2018-unsupervised, artetxe2017unsupervised, lachaux2020unsupervised} to solve this problem. For example, \citet{gulcehre2015using} proposed integrating a Language model into the decoder. \citet{xia2016dual} proposed Neural MT (NMT) as a bidirectional and dual learning task. More recent advancements in unsupervised MT leverages back-translation (BT)~\cite{sennrich-etal-2016-improving, lample2018unsupervised, lample-etal-2018-phrase}. 
In back-translation, the target-to-source model generates noisy sources given target sequences and then trains the source-to-target model to reconstruct the targets and vice versa. 
While BT has been widely adopted for unsupervised NMT, it is used in other applications \cite{zhu2017unpaired, pmlr-v80-hoffman18a, shen2017style, yang2018unsupervised, zhang2018style}.


% in cycle-consistency \cite{zhu2017unpaired, pmlr-v80-hoffman18a} and style transfer \cite{shen2017style, yang2018unsupervised, zhang2018style}.









==> [EACL 2023] Summarize Generate to Backtranslate/sections/7_conclusion.tex <==
\section{Conclusion}
In this research, we show that pre-trained sequence-to-sequence models ({\em e.g.}, PLBART) are not suitable for direct adaptation via back-translation to learn to translate. 
% Due to the lack of knowledge about cross-lingual generation, such models cannot generate code in the source language given an input code in the target language.
% , which is a crucial step in back-translation. 
% As a solution to this problem, we propose to use code summarization and generation as an alternative to target-to-source translation in the back-translation approach. 
To address the issue, we propose to use code summarization and generation as an alternative to performing back-translation. 
% We leverage \emph{bimodal} data, e.g., source code and their summaries, to train a code-to-summary and a summary-to-code generation model. Subsequently, these models are used to generate target-to-summary and summary-to-source, which is equivalent to target-to-source translation, enabling training pre-trained programming language models via back-translation.
We show that our proposed approach turns PLBART into a translation model that performs competitively to existing unsupervised translation models.

\section*{Limitations}
One of the risks of using our developed translation model is that we used the Github dataset for training that may contain information that uniquely identifies an individual or offensive content.
Since we are developing the translation model for research purposes \emph{only}, we believe our usage of the Github data does not violate their licensing terms and conditions.
While we do not present it as a justification, the PLBART model was pre-trained on the Github data that may include sensitive information.
As we converted PLBART into a programming language translation model, it is unlikely to generate sensitive information unless it is provided such information as input. However, we should be careful while using translation models trained using unfiltered data.
All the experiments performed in this work are based only on one seed. Therefore, using other random seeds may lead to results that could be different from ours.


\section*{Ethics Statement}
\paragraph{Training data and its risks} 
We use the GitHub public dataset available on Google BigQuery filtered to keep only projects with open-source licenses.\footnote{We select the open-source licenses: `apache-2.0', `mit', `gpl-2.0', `gpl-3.0', `bsd-2-clause', `bsd-3-clause'.}
While we do not perform preprocessing that would eliminate any personally identifiable information or offensive content, we remove natural language comments that presumably reduce toxic content. 
Nonetheless, using code language models (LMs) comes with certain risks, e.g., generating biased, toxic, and vulnerable code. \citet{chen2021evaluating} discussed the broader impact and risks of code LMs (Section 7). We should keep those factors to ensure the responsible use of code LMs.


\paragraph{Carbon Footprint} We avoided using large models, reducing their environmental impacts. We train \texttt{PLBART-base} model on summarization-generation and backtranslation for a maximum of 10k steps on 8 \texttt{RTX 2080 Ti} GPUs that took 1-2 days. Therefore, the training would emit approximately 15kg of carbon into the environment.\footnote{Calculated using \url{https://mlco2.github.io/impact}, based on a total of 200 hours of training on RTX 2080 Ti and Amazon Web Services as the provider.} No model finetuning is performed in this work.



==> [EACL 2023] Summarize Generate to Backtranslate/table/1_data_stat.tex <==
\begin{table}[t]
\centering
% \resizebox{\linewidth}{!}
{%
% \small
\begin{tabular}{l r r}
\hline
 & Java & Python \\ 
\hline
\multicolumn{3}{l}{Github - \emph{unimodal} data} \\
\cdashline{1-3}
% Nb of functions & 44.5 M & 42.0 M \\
% Nb of tokens & 3.3 B & 4.1 B \\
Nb of functions & 7.2 M & 8.3 M \\
Nb of tokens & 752 M & 665 M \\
\hline
\multicolumn{3}{l}{CodeNet - \emph{unimodal} data} \\
\cdashline{1-3}
Nb of functions & 0.42 M & 0.15 M \\
Nb of tokens & 47.3 M & 17.0 M \\
\hline
\multicolumn{3}{l}{CodeXGlue - \emph{bimodal} data} \\
\cdashline{1-3}
Nb of functions & 164,923 & 251,818 \\
Nb of tokens & 21.2 M & 44.3 M \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
Statistics of the data used to train PLBART at different stages in this work. \emph{Bimodal} data refers to parallel function-summary pairs, while \emph{unimodal} data refers to monolingual (and unparallel) functions.
}
\label{table:data_stat}
% \vspace{-2mm}
\end{table}



==> [EACL 2023] Summarize Generate to Backtranslate/table/2_main_result.tex <==
\begin{table*}[!ht]
\centering
\resizebox{\linewidth}{!}
{%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{l|c c c c|c c c c}
% \begin{tabular}{@{}l@{\hskip 0.05in} | c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.1in} c@{\hskip 0.1in} | c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.1in} c@{\hskip 0.1in}}
\hline
\multirow{2}{*}{{Models}} & \multicolumn{4}{c|}{{Java $\rightarrow$ Python}} & \multicolumn{4}{c}{{Python $\rightarrow$ Java}} \\ 
\cline{2-9}
& BLEU  & EM & CodeBLEU & CA & BLEU & EM & CodeBLEU & CA  \\ 
\hline
j2py* & - & - & - & 38.3 & - & - & - & - \\
% TransCoder$^\ast$ & 68.1 & 3.7 & - & 35.0 & 64.6 & 0.8 & - & 24.7 \\
TransCoder$^\ast$ & 68.1 & 3.7 & - & 46.9 & 64.6 & 0.8 & - & 32.6 \\
TransCoder w/ DOBF$^\ast$ & - & - & - & 49.2 & - & - & - & 40.4 \\
% \cdashline{1-9}
\hdashline
\sng \eqref{eq:mulsumgen} & 7.6 & 0.0 & 15.8 & 0.2 & 12.4 & 0 & 16.3 & 0.2 \\
% TransCoder & 67.6 & 1.9 & 65.6 & 47.0 & 65.0 & 0.6 & 70.3 & 32.6 \\
% DOBF & {\bf 71.4} & {\bf 3.5} & {\bf 67.4} & {\bf 49.1} & {\bf 66.3} & {\bf 1.8} & {\bf 70.4} & 39.6 \\
\cdashline{1-9}
\multicolumn{9}{l}{PLBART \bf{(this work)}} \\
\cdashline{1-9}
\hdashline
trained via BT & 31.2 & 0.0 & 36.6 & 0.0 & 31.7 & 0.0 & 32.1 & 0.0 \\
trained via BT (via \sng) & 64.2 & 2.8 & 63.4 & 40.4 & 64.1 & 2.1 & 65.9 & 31.9 \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
Evaluation results of the baselines models and our proposed framework using greedy decoding. $^\ast$ indicates the updated scores reported in the official code repository of \citet{lachaux2020unsupervised}. 
Note that, TransCoder and PLBART models have 312M and 140M parameters, respectively.
}
\label{table:main_result}
% \vspace{-2mm}
\end{table*}



==> [EACL 2023] Summarize Generate to Backtranslate/table/3_beam_result.tex <==
% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}
% {%
% % \small%
% % \def\arraystretch{1.05}%
% \begin{tabular}{l|c@{\hskip 0.1in} c}
% \hline
% Models & Java $\rightarrow$ Python & Python $\rightarrow$ Java \\ 
% \hline
% \multicolumn{3}{l}{\emph{TransCoder}} \\
% \cdashline{1-3}
% CA@1 k=1 & 35.0 & 35.5 \\
% CA@1 k=10 & 49.0 & 38.4 \\
% CA@5 k=5 & 60.0 & 47.0 \\
% CA@10 k=10 & 64.4 & 50.0 \\
% \cdashline{1-3}
% \multicolumn{3}{l}{\emph{PLBART}} \\
% \cdashline{1-3}
% CA@1 k=1 & 24.7 & 43.8 \\
% CA@1 k=10 & 36.6 & 45.4 \\
% CA@5 k=5 & 44.3 & 52.5 \\
% CA@10 k=10 & 51.1 & 55.0 \\
% \hline
% \end{tabular}
% }
% % \vspace{-2mm}
% \caption{
% Write caption.
% }
% \label{table:beam_result}
% % \vspace{-2mm}
% \end{table}

\begin{table}[!ht]
\centering
% \resizebox{\linewidth}{!}
{%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{l|c@{\hskip 0.1in} c}
\hline
Models & TransCoder & PLBART \\ 
\hline
\multicolumn{3}{l}{\emph{Java $\rightarrow$ Python}} \\
\cdashline{1-3}
CA@1 B=1 & 46.9 & 40.4 \\
CA@1 B=10 & 48.8 & 41.8 \\
CA@5 B=5 & 60.0 & 47.7 \\
CA@10 B=10 & 64.4 & 50.3 \\
\cdashline{1-3}
\multicolumn{3}{l}{\emph{Python $\rightarrow$ Java}} \\
\cdashline{1-3}
CA@1 B=1 & 32.6 & 31.9 \\
CA@1 B=10 & 36.0 & 34.5 \\
CA@5 B=5 & 44.3 & 45.1 \\
CA@10 B=10 & 51.1 & 50.0 \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
Computational accuracy (CA@m) with beam search decoding and comparison between TransCoder and PLBART. TransCoder's performances are reported from \citet{lachaux2020unsupervised}. 
The value B indicates the beam size. 
CA@m B=n means that we use beam decoding to generate n translations, and select the top m translations based on their log-probability scores. 
}
\label{table:beam_result}
% \vspace{-2mm}
\end{table}



==> [EACL 2023] Summarize Generate to Backtranslate/table/4_comp_acc.tex <==
% \begin{table}[!ht]
% \centering
% % \resizebox{\linewidth}{!}
% {%
% % \small%
% % \def\arraystretch{1.05}%
% \begin{tabular}{l | c@{\hskip 0.1in} c@{\hskip 0.1in} c}
% \hline
% & TransCoder & DOBF & PLBART \\
% \hline
% \multicolumn{3}{l}{\emph{Java $\rightarrow$ Python}} \\
% \cdashline{1-4}
% \#tests & 464 & 464 & 464 \\
% Error & 149 & {\bf 136} & 146 \\
% Failure & 93 & {\bf 91} & 146 \\
% Success & 218 & {\bf 228} & 164 \\
% EM & 17 & {\bf 26} & 24 \\
% Timeout & {\bf 4} & 9 & 8 \\
% \cdashline{1-4}
% \multicolumn{4}{l}{\emph{Python $\rightarrow$ Java}} \\
% \cdashline{1-4}
% \#tests & 482 & 482 & 482 \\
% Error & 201 & {\bf 188} & 212 \\
% Failure & 118 & 98 & {\bf 53} \\
% Success & 157 & 191 & {\bf 211} \\
% EM & 6 & {\bf 14} & 2 \\
% Timeout & 6 & {\bf 5} & 6 \\
% \hline
% \end{tabular}
% }
% % \vspace{-2mm}
% \caption{
% Breakdown of the computational performances on evaluation set for Java--Python translation. 
% }
% \label{table:comp_acc}
% % \vspace{-2mm}
% \end{table}


\begin{table}[!ht]
\centering
% \resizebox{\linewidth}{!}
{%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{l |c c}
\hline
& TransCoder & PLBART \\
\hline
\multicolumn{3}{l}{\emph{Java $\rightarrow$ Python}} \\
\cdashline{1-3}
\#Tests & 464 & 464 \\
Error & 149 & 146 \\
Failure & 93 & 123 \\
Success & 218 & 188 \\
\quad EM & 17  & 24 \\
Timeout & 4 & 7 \\
\cdashline{1-3}
\multicolumn{3}{l}{\emph{Python $\rightarrow$ Java}} \\
\cdashline{1-3}
\#Tests & 482 & 482 \\
Error & 201 & 212 \\
Failure & 118 & 108 \\
Success & 157 & 154 \\
\quad EM & 6 & 2 \\
Timeout & 6 & 8 \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
Detailed results of computational accuracy using greedy decoding for Java $\leftrightarrow$ Python translation. 
}
\label{table:comp_acc}
% \vspace{-2mm}
\end{table}


==> [EACL 2023] Summarize Generate to Backtranslate/table/5_error_breakdown.tex <==
% \begin{table*}[!ht]
% \centering
% % \resizebox{\linewidth}{!}
% {%
% % \small%
% % \def\arraystretch{1.05}%
% \begin{tabular}{l c c c c c c}
% \hline
% \multirow{2}{*}{Error Category} & \multicolumn{3}{c}{Java to Python} & \multicolumn{3}{c}{Python to Java} \\ 
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% & TransCoder  & DOBF & PLBART & TransCoder & DOBF & PLBART  \\ 
% % \hline
% \midrule
% \rowcolor{dark-gray}
% Total & 149 & 136 & 146 & 201 & 188 & 212 \\
% \midrule
% \rowcolor{light-gray}
% Compilation Errors & 0 & 0 & 0 & 151 & 144 & 180 \\
% \quad Syntax error  & - & - & - & ? & ? & ? \\
% \quad Type error  & - & - & - & ? & ? & ? \\
% \quad Cant find symbol  & - & - & - & ? & ? & ? \\
% \quad Bad operand  & - & - & - & ? & ? & ? \\
% \quad Others  & - & - & - & ? & ? & ? \\
% \midrule
% \rowcolor{light-gray}
% Runtime Errors & 149 & 136 & 146 & 50 & 43 & 27 \\
% \quad SyntaxError  & ? & ? & ? & ? & ? & ? \\
% \quad TypeError  & ? & ? & ? & ? & ? & ? \\
% \quad NameError  & ? & ? & ? & ? & ? & ? \\
% \quad UnboundLocalError  & ? & ? & ? & ? & ? & ? \\
% \quad AttributeError  & ? & ? & ? & ? & ? & ? \\
% \quad ZeroDivisionError  & ? & ? & ? & ? & ? & ? \\
% \quad IndexError  & ? & ? & ? & ? & ? & ? \\
% \quad RecursionError  & ? & ? & ? & ? & ? & ? \\
% \quad KeyError  & ? & ? & ? & ? & ? & ? \\
% \quad ValueError  & ? & ? & ? & ? & ? & ? \\
% \quad OverflowError  & ? & ? & ? & ? & ? & ? \\
% \hline
% \end{tabular}
% }
% % \vspace{-2mm}
% \caption{
% Write a caption.
% }
% \label{table:main_result}
% % \vspace{-2mm}
% \end{table*}


% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}
% {%
% % \small%
% % \def\arraystretch{1.05}%
% \begin{tabular}{l@{\hskip 0.1in} c@{\hskip 0.1in} c@{\hskip 0.1in} c}
% \hline
% Error Category & TransCoder & DOBF & PLBART  \\ 
% \midrule
% \rowcolor{dark-gray}
% Total Errors & 149 & 136 & 146 \\
% \midrule
% \rowcolor{light-gray}
% Compilation & 0 & 0 & 0 \\
% \midrule
% \rowcolor{light-gray}
% Runtime & 149 & 136 & 146 \\
% \quad Attribute & 11 & 23 & 5 \\
% \quad Index  & 18 & 24 & 20 \\
% \quad Key  & 3 & 2 & 4 \\
% \quad Name  & 17 & 12 & 16 \\
% \quad Overflow  & 2 & 1 & 1 \\
% \quad Recursion  & 1 & 2 & 2 \\
% \quad Syntax & 26 & 6 & 9 \\
% \quad Type  & 47 & 38 & 61 \\
% \quad UnboundLocal & 13 & 12 & 11 \\
% \quad Value  & 11 & 14 & 15 \\
% \quad ZeroDivision & 0 & 2 & 2 \\
% \hline
% \end{tabular}
% }
% \caption{
% Java to Python (based on greedy search).
% }
% \label{table:main_result}
% % \vspace{-2mm}
% \end{table}


\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}
{%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{l@{\hskip 0.1in} c@{\hskip 0.1in} c}
\hline
Error Category & TransCoder & PLBART  \\ 
\midrule
\rowcolor{dark-gray}
\#Errors (Java $\rightarrow$ Python)  & 149 & 146 \\
\midrule
\rowcolor{light-gray}
Compilation & - & - \\
\midrule
\rowcolor{light-gray}
Runtime & 149 & 146 \\
\quad TypeError  & 47 & 61 \\
\quad IndexError  & 18 & 20 \\
\quad NameError  & 17 & 16 \\
\quad ValueError  & 11 & 15 \\
\quad UnboundLocalError & 13 & 11 \\
\quad Others & 17 & 14 \\
\quad SyntaxError & 26 & 9 \\
\midrule
\rowcolor{dark-gray}
\#Errors (Python $\rightarrow$ Java) & 201 & 212 \\
\midrule
\rowcolor{light-gray}
Compilation & 151 & 180 \\
\quad TypeError  & 89 & 108 \\
\quad CantFindSymbol  & 23 & 30 \\
\quad SyntaxError  & 14 & 25 \\
\quad BadOperand  & 15 & 12 \\
\quad Others & 10 & 5 \\
\midrule
\rowcolor{light-gray}
Runtime & 50 & 27 \\
\quad IndexOutOfBoundsE.  & 40 & 15 \\
\quad NumberFormatE.  & 5 & 6 \\
\quad NullPointerE.  & 2 & 3 \\
\quad Others & 3 & 3 \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
Category of errors made by the TransCoder and PLBART translation models. 
The error categories are sorted based on the PLBART's error count on the respective category. 
In Python $\rightarrow$ Java runtime error categories, ``E.'' stands for ``Exception''.
% A detailed categorization is provided in the Appendix.
}
\label{table:errors_made_by_model}
% \vspace{-2mm}
\end{table}



==> [EACL 2023] Summarize Generate to Backtranslate/table/6_error_analysis.tex <==
\begin{table*}[!ht]
% \setlength{\tabcolsep}{0.2em}
\centering
% \resizebox{\linewidth}{!}
% {%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{p{11cm} c}
\hline
Error Category & Count  \\ 
\midrule
\rowcolor{light-gray}
Type Error & 61 \\
list indices must be integers or slices, not {\bf A} & 18 \\
{\bf A} object does not support item assignment & 13 \\
{\bf A} object cannot be interpreted as an integer & 8 \\
unsupported/bad operand type(s) & 10 \\
int object is not iterable/callable/subscriptable & 6 \\
Others & 6 \\
\midrule
\rowcolor{light-gray}
Index Error & 20 \\
{\bf B} index out of range & 19 \\
others & 1 \\
\midrule
\rowcolor{light-gray}
Name Error & 16 \\
name {\bf C} is not defined & 16 \\
\midrule
\rowcolor{light-gray}
Value Error & 15 \\
not enough values to unpack & 7 \\
too many values to unpack & 3 \\
the truth value of an array with more than one element is ambiguous & 3 \\
others & 2 \\
\midrule
\rowcolor{light-gray}
Unbound Local Error & 11 \\
local variable {\bf D} referenced before assignment & 11 \\
\hline
\end{tabular}
% }
% \vspace{-2mm}
\caption{
Analyzing the five most frequent error cases (123 out of 146) encountered in PLBART generated Java to Python translation.
{\bf A} and {\bf B} indicate \{bool, int, tuple, str, range\} and \{string, list\}, respectively. {\bf C} and {\bf D} indicate identifier (class, function, variable) names.
}
\label{table:error_analysis_plbart_top_errors}
% \vspace{-2mm}
\end{table*}






==> [EACL 2023] Summarize Generate to Backtranslate/table/7_data_impact.tex <==
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}
{%
% \small%
% \def\arraystretch{1.05}%
\begin{tabular}{l|c c c c|c c c c}
\hline
\multirow{ 2}{*}{{Data Source}} & \multicolumn{4}{c|}{{Java to Python}} & \multicolumn{4}{c}{{Python to Java}} \\ 
\cline{2-9}
& BLEU  & EM & CodeBLEU & CA & BLEU & EM & CodeBLEU & CA  \\ 
\hline
Github & 64.2 & 2.8 & 63.4 & 40.4 & 64.1 & 2.1 & 65.9 & 31.9 \\
CodeNet & 65.6 & 3.1 & 64.7 & 50.9 & 65.1 & 2.5 & 68.5 & 46.5 \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{
PLBART evaluation results when our proposed framework uses data from Github (available via BigQuery \cite{hoffa2016github}) and competitive programming sites (available via CodeNet \cite{puri2021project}).
}
\label{table:data_impact}
% \vspace{-2mm}
\end{table*}


